Langevin Monte Carlo without smoothness

Langevin Monte Carlo (LMC) is an iterative algorithm used to generate samples from a distribution that is known only up to a normalizing constant. The nonasymptotic dependence of its mixing time on the dimension and target accuracy is understood mainly in the setting of smooth (gradient-Lipschitz) log-densities, a serious limitation for applications in machine learning. In this paper, we remove this limitation, providing polynomial-time convergence guarantees for a variant of LMC in the setting of nonsmooth log-concave distributions. At a high level, our results follow by leveraging the implicit smoothing of the log-density that comes from a small Gaussian perturbation that we add to the iterates of the algorithm and controlling the bias and variance that are induced by this perturbation.

==> stochasticgradients.tex <==
We analyze the convergence of Langevin diffusion in the \emph{total-variation} distance for target distributions of the form $p^* \propto e^{-\bar{U}(\vx_t)},$ where $\bar{U}(\cdot) = U(\cdot) + \psi(\cdot)$, $U(\cdot)$ is $M$-smooth, and $\psi(\cdot)$ is $m$-smooth and $\lambda$-strongly convex. 
%
To analyze the convergence, we first need to bound  the discretization error. Consider the first process which describes the exact continuous time process,
\begin{align}\label{def:continuousprocess}
    \dd\vx_t = - \nabla \bar{U}(\vx_t) \dd t + \sqrt{2}\dd\mB_t,
\end{align}
with initial condition $\vx_0 \sim  \nu$. Let the distribution of $\vx_t$ be denoted by $p_t$. Let $\nu \mathbb{P}_t$ denote the distribution of the entire path $\{\vx_s\}_{s=0}^t$. Consider a second process that describes the Euler-Mayurama discretization of \eqref{def:continuousprocess},
\begin{align}
    \label{def:discreteprocess}
    \dd{\tilde{\vx}}_t = -\vb_t(\tilde{\vx}_t) \dd t + \sqrt{2}\dd \mB_t,
\end{align}
with the same initial condition $\bf{\tilde{x}}_0  \sim \nu$ and $\vb(\tilde{\vx}_t) = \sum_{k=0}^{\infty}\hat{\nabla} \bar{U}(\tilde{\vx}_{k\eta})\cdot \mathbb{I}\left[t\in [k\eta,(k+1)\eta)\right]$. Here $\hat{\nabla}\bar{U}(y)$ is an \emph{unbiased} stochastic gradient of $\bar{U}$ at $y \in \mathbb{R}^d$ with variance bounded by $\sigma^2d$. Let the distribution of $\tilde{\vx}_t \sim \tilde{p}_t$ and let $\nu\tilde{\mathbb{P}}_t$ denote the distribution of the entire stochastic process $\{\tilde{\vx}_s\}_{s=0}^t$. Similar to \cite{dalalyan2017theoretical} we use Girsanov's formula \cite[Chapter 8]{oksendal2003stochastic} to control the Kullback-Leibler divergence between the distributions $\nu\mathbb{P}_t$ and $\nu\tilde{\mathbb{P}}_t$.
\begin{align}\label{def:girsanovformula}
    KL\left(\nu \mathbb{P}_t \lvert \nu \tilde{\mathbb{P}}_t\right)  = \frac{1}{4} \int_{0}^t\mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_s) - \vb(\tilde{\vx}_s) \rv_2^2\right]ds.
\end{align}

\begin{lemma}[Discretization Error Bound] \label{lem:discretebound}Let $\mathbf{x}^*$ be a point such that $\nabla \bar{U}(\mathbf{x}^*) = 0$. If $\eta < 1/(2(M+m))$, then for any integer $K\ge 1$ we have,
\begin{align*}
     KL\left(\nu\mathbb{P}_{K\eta} \lvert \nu \tilde{\mathbb{P}}_{K\eta}\right) & \le \frac{(M+m)^3\eta^2}{9} \mathbb{E}_{y\sim \nu}\left[\lv y - \vx^* \rv_2^2\right]+\frac{(M+m)^2Kd\eta^3}{9}+\frac{(M+m)^2Kd\eta^2}{2} + \frac{K\eta \sigma^2 d}{2}.
\end{align*}
\end{lemma}
\begin{proof} By Girsanov's formula Eq. \eqref{def:girsanovformula} and the definition of $\vb(\tilde{\vx})$ we have,
\begin{align*}
     KL\left(\nu\mathbb{P}_{K\eta} \lvert \nu \tilde{\mathbb{P}}_{K\eta}\right) & =  \frac{1}{4}\int_{0}^{K\eta} \mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_s) - \vb(\tilde{\vx}_s) \rv_2^2\right]ds \\
    & = \frac{1}{4} \sum_{k=0}^{K-1} \int_{k\eta}^{(k+1)\eta} \mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_s) - \hat{\nabla} \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] ds\\
& \le \frac{1}{2} \sum_{k=0}^{K-1} \int_{k\eta}^{(k+1)\eta} \mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_s) - \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] ds    + \frac{1}{2} \sum_{k=0}^{K-1} \int_{k\eta}^{(k+1)\eta} \mathbb{E}\left[\lv \hat{\nabla} \bar{U}(\tilde{\vx}_s) - \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] ds,    \\
& \le \frac{1}{2} \sum_{k=0}^{K-1} \int_{k\eta}^{(k+1)\eta} \mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_s) - \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] ds + \frac{K\eta \sigma^2 d}{2}.
\end{align*}
where the last step follows by Young's inequality.
By using the smoothness of $\bar{U}$ we get,
\begin{align}
    \nonumber  KL\left(\nu\mathbb{P}_{K\eta} \lvert \nu \tilde{\mathbb{P}}_{K\eta}\right) & \le \frac{(M+m)^2}{2} \sum_{k=0}^{K-1} \int_{k\eta}^{(k+1)\eta} \mathbb{E}\left[\lv  \tilde{\vx}_s -  \tilde{\vx}_{k\eta}\rv_2^2\right] ds + \frac{K\eta \sigma^2 d}{2}. \label{eq:discretizationboundfirstpart}
\end{align}
Let us unpack and bound the first term on the right hand side. By definition of $\tilde{\vx}_s$ we get, for each $k \in \{0,\ldots, K-1\}$,
\begin{align*}
      \int_{k\eta}^{(k+1)\eta} \mathbb{E}\left[\lv  \tilde{\vx}_s -  \tilde{\vx}_{k\eta}\rv_2^2\right] ds&  =  \int_{k\eta}^{(k+1)\eta} \mathbb{E}\left[\left\lv  \int_{k\eta}^{s}\left(\nabla \bar{U}(\tilde{\vx}_{k\eta})+\sqrt{2}\dd \mB_r\right)dr\right\rv_2^2\right] ds \\
      & = \int_{k\eta}^{(k+1)\eta} \left(\mathbb{E}\left[\left\lv\nabla \bar{U}(\tilde{\vx}_{k\eta})\right\rv_2^2(s-k\eta)^2\right]+2d(s-k\eta)\right)ds,
\end{align*}
plugging this back into Eq. \eqref{eq:discretizationboundfirstpart} we get,
\begin{align*}
     KL\left(\nu\mathbb{P}_{K\eta} \lvert \nu \tilde{\mathbb{P}}_{K\eta}\right) &\le \frac{(M+m)^2\eta^3}{6}\sum_{k=0}^{K-1}\mathbb{E}\left[\left\lv\nabla \bar{U}(\tilde{\vx}_{k\eta})\right\rv_2^2\right] + \frac{dK(M+m)^2\eta^2}{2} + \frac{K\eta \sigma^2 d}{2}.
\end{align*}
By invoking Lemma \ref{lem:gradientbound} we get the desired result.
\end{proof}

\begin{lemma}\label{lem:gradientbound} Let $\eta \le 1/(2(M+m))$. Let $K \ge 1$ be an integer then,
\begin{align*}
    \eta \sum_{k=0}^{K-1} \mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] \le \frac{2(M+m)}{3}\mathbb{E}\left[\lv \tilde{\vx}_0 - \vx^* \rv_2^2\right] + \frac{4(M+m)K\eta d}{3} .
\end{align*}
\end{lemma}
\begin{proof} Let $\bar{U}^{(k)} := \bar{U}(\tilde{\vx}_{k\eta})$ then by the smoothness of $\bar{U}$ (Eq. \eqref{eq:inexact-grad-model}) we get,
\begin{align*}
    \bar{U}^{(k+1)} &\le \bar{U}^{(k)} + \langle \nabla \bar{U}(\tilde{\vx}_{k\eta}),\tilde{\vx}_{(k+1)\eta} - \tilde{\vx}_{k\eta}\rangle + \frac{M+m}{2}\left\lv \tilde{\vx}_{(k+1)\eta} - \tilde{\vx}_{k\eta}\right\rv_2^2\\
    & = \bar{U}^{(k)} - \eta \lv \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2 + \sqrt{2\eta}\langle  \nabla \bar{U}(\tilde{\vx}_{k\eta}),\vg_k\rangle + \frac{M+m}{2}\left\lv \eta  \nabla \bar{U}(\tilde{\vx}_{k\eta}) -\sqrt{2\eta}\vg_k \right\rv_2^2 ,
\end{align*}
where $\vg_k = \int_{s=k\eta}^{(k+1)\eta} \dd \mB_s$, is independent Gaussian noise. Taking expectations on both sides we get,
\begin{align*}
    \mathbb{E}\left[\bar{U}^{(k+1)}\right] & \le \mathbb{E}\left[\bar{U}^{(k)}\right] -\eta \mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] + \frac{M+m}{2}\eta^2\mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] + (M+m)\eta d \\
    & = \mathbb{E}\left[\bar{U}^{(k)}\right]  -\eta\left(1-\frac{(M+m)\eta}{2}\right)\mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right]+ (M+m)\eta d .
\end{align*}
Rearranging the above inequality and summing from $k=0$ to $K-1$ we get that,
\begin{align*}
    \eta \sum_{k=0}^{K-1} \mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] &\le \frac{4}{3}\mathbb{E}\left[\bar{U}^{((0))} - \bar{U}^{(K)}\right] + \frac{4(M+m)K\eta d}{3} .
\end{align*}
Let $\bar{U}^* = \inf_{\vx \in \mathbb{R}^d}\bar{U}(\vx)$. Therefore we have $\bar{U}^{K} \ge \bar{U}^*$ and $\bar{U}^{(0)} - \bar{U}^* \le (M+m)\lv \tilde{\vx}_0 - \vx^* \rv_2^2/2 $. Combining this with the inequality above we get,
\begin{align*}
    \eta \sum_{k=0}^{K-1} \mathbb{E}\left[\lv \nabla \bar{U}(\tilde{\vx}_{k\eta})\rv_2^2\right] &\le \frac{2(M+m)}{3}\mathbb{E}\left[\lv \tilde{\vx}_0 - \vx^* \rv_2^2\right] + \frac{4(M+m)K\eta d}{3} .
\end{align*}
\end{proof}

\begin{theorem} Let the initial point be drawn from a Normal distribution $\tilde{\vx}_0 \sim \nu = N (\vx^*, (M+m)^{-1}I_{d\times d})$, where $\vx^*$ is a point such that $\nabla \bar{U}(\vx^*) = 0$. Let the step size $\eta < 1/(2(M+m))$. Then for any integer $K\ge 1$ we have,
\begin{align*}
    \lv p_{K\eta} -p^*\rv_{TV} &\le \frac{1}{2}\exp\left(\frac{d}{4}\log\left(\frac{M+m}{m}\right)-\frac{K\eta m}{2}\right) + (M+m)\eta\sqrt{\frac{d}{18}} +(M+m)\sqrt{\frac{Kd\eta^3}{18}}\\ & \qquad \qquad \qquad \qquad +(M+m)\eta\sqrt{\frac{Kd}{2}} + \sqrt{\frac{\delta \eta K M}{2}}.
\end{align*}
\end{theorem}
\begin{proof}
By applying triangle inequality to total variation distance we have,
\begin{align*}
    \lv \tilde{p}_{K\eta} - p^* \rv_{TV} &\le \lv p_{K\eta} - p^* \rv_{TV} + \lv \tilde{p}_{K\eta} - p_{K\eta} \rv_{TV}.
\end{align*}
We start off by choosing the initial distribution to be a Gaussian $\tilde{\vx}_0 \sim N(\vx^*,(M+m)^{-1}I_{d\times d})$. Therefore by \cite[Lemma 5]{dalalyan2017theoretical} we have that the first term, \todo{correct the continuous contraction claim.
}
\begin{align*}
    \lv p_{K\eta} - p^* \rv_{TV} &\le \frac{1}{2}\exp\left(\frac{d}{4}\log\left(\frac{M+m}{m}\right)-\frac{K\eta m}{2}\right).
\end{align*}
While by Lemma \ref{lem:discretebound} which holds for a fixed initial point $x$ combined with the convexity of KL-divergence we get that,
\begin{align*}
    \lv \tilde{p}_{K\eta} - p_{K\eta} \rv_{TV} &\le
    \lv \nu\mathbb{P}_{K\eta} - \nu \tilde{\mathbb{P}}_{K\eta} \rv_{TV} \le  \left( \frac{1}{2}KL\left(\nu\mathbb{P}_{K\eta} \lvert \nu \tilde{\mathbb{P}}_{K\eta}\right)\right)^{1/2}\\
    & \le \sqrt{\frac{(M+m)^{3}\eta^2}{18} \mathbb{E}_{y\sim p_{0}}\left[\lv y - \vx^* \rv_2^2\right]}+\sqrt{\frac{(M+m)^2Kd\eta^3}{18}}\\ & \qquad \qquad \qquad \qquad +\sqrt{\frac{(M+m)^2Kd\eta^2}{2}} + \sqrt{\frac{K\sigma^2 d \eta}{2}},
\end{align*}
where the first inequality is by data-processing inequality and the second is by Pinsker's inequality. It is a simple calculation to show that $\mathbb{E}_{y\sim p_{0}}\left[\lv y - \vx^* \rv_2^2\right] = d/(M+m)$.
Combining this with the inequality above yields the desired claim.
\end{proof}

\begin{corollary}
State corollary with chosen values of $\eta,\delta, M, K$
\end{corollary}
\begin{proof}
Fill this up when it is clear what is better, using Gaussian smoothing or without using Gaussian smoothing.
\end{proof}
